Knowledge Distillation via the Target-aware Transformer

Knowledge distillation becomes a de facto standard to improve the performance of small neural networks. Most of the previous works propose to regress the representational features from the teacher to the student in a one-to-one spatial matching fashion. However, people tend to overlook the fact that, due to the architecture differences, the semantic information on the same spatial location usually vary. This greatly undermines the underlying assumption of the one-to-one distillation approach. To this end, we propose a novel one-to-all spatial matching knowledge distillation approach. Specifically, we allow each pixel of the teacher feature to be distilled to all spatial locations of the student features given its similarity, which is generated from a target-aware transformer. Our approach surpasses the state-of-the-art methods by a significant margin on various computer vision benchmarks, such as ImageNet, Pascal VOC and COCOStuff10k. Code is available at https://github.com/sihaoevery/TaT.

==> tex/tables/ablation-parametric.tex <==

%----------------------------------------------------------------------------
\begin{table}[h]
    \centering
    \caption{\textbf{Comparing the semantic segmentation results (in mIoU\%) of different methods on COCOStuff10k.}
    As most baselines do not provide the code on the COCO dataset except KR, we only compare our method to KR in this case. We reproduce the baseline using the official code with the same training procedure. Our method surpasses the baseline by nearly 2\%, and further demonstrate the effectiveness of our approach.
    }
    \vspace{-2mm}
    {\tablestyle{8pt}{1.1}
    \begin{tabular}{@{}l|cccc@{}}
    \toprule
        &Sutdent   &KR~\cite{chen2021distilling}&Our &Teacher  \\
        \midrule
        ResNet18    &26.33 &26.73 &\textbf{28.75} &33.10 \\
        MobilenetV2 &26.29 &26.63 &\textbf{28.05}  &33.10 \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:seg_coco}
    \vspace{-3mm}
\end{table}
%----------------------------------------------------------------------------

%--------------------------------------------------------------------------
\begin{table}[t!]
\centering
\caption{\textbf{Impact of function $\theta(\cdot)$ on a variety of network architectures.} We report the top-1 accuracy on Cifar-100. $id$ indicates for identity mapping.  }
\vspace{-2mm}
{
\begin{tabular}{@{}ll|cc@{}}
    \toprule
    Teacher  &Student &Conv+BN & $id$  \\ 
    % \hline
    \midrule
    ResNet56 &ResNet20  &71.45 &\textbf{71.59} \\
    ResNet110 &ResNet20 &71.68 & \textbf{71.70} \\
    ResNet110 &ResNet32 &73.75 &\textbf{74.05}\\
    ResNet32$\times$4 &ResNet8$\times$4 &75.30 &7\textbf{5.89}\\
    VGG13 &VGG8 &73.48 &\textbf{74.39}\\
    \bottomrule
\end{tabular}
}
\label{tab:cifar_1x1}
\vspace{-4mm}
\end{table}
